Multi-Player Zero-Sum Markov Games with Networked Separable Interactions

We study a new class of Markov games, \emph(multi-player) zero-sum Markov Games} with \emph{Networked separable interactions} (zero-sum NMGs), to model the local interaction structure in non-cooperative multi-agent sequential decision-making. We define a zero-sum NMG as a model where {the payoffs of the auxiliary games associated with each state are zero-sum and} have some separable (i.e., polymatrix) structure across the neighbors over some interaction network. We first identify the necessary and sufficient conditions under which an MG can be presented as a zero-sum NMG, and show that the set of Markov coarse correlated equilibrium (CCE) collapses to the set of Markov Nash equilibrium (NE) in these games, in that the product of per-state marginalization of the former for all players yields the latter. Furthermore, we show that finding approximate Markov \emph{stationary} CCE in infinite-horizon discounted zero-sum NMGs is \texttt{PPAD}-hard, unless the underlying network has a ``star topology''. Then, we propose fictitious-play-type dynamics, the classical learning dynamics in normal-form games, for zero-sum NMGs, and establish convergence guarantees to Markov stationary NE under a star-shaped network structure. Finally, in light of the hardness result, we focus on computing a Markov \emph{non-stationary} NE and provide finite-iteration guarantees for a series of value-iteration-based algorithms. We also provide numerical experiments to corroborate our theoretical results.

==> main6-OMWU.tex <==
\section{Non-Stationary NE Computation}
\label{section:OMWU}

We now focus on computing an (approximate)  Markov \emph{non-stationary} equilibrium in MZNMGs.  
In particular, {we show that when relaxing the stationarity requirement, not only CCE, but NE, can be computed efficiently.}  Before introducing our algorithm, we first recall the folklore result that approximating Markov non-stationary NE in \emph{infinite-horizon} discounted settings can be achieved by finding approximate Markov NE in \emph{finite-horizon} settings, with a large enough horizon length (c.f. \Cref{prop:truncation}). Hence, we will focus on the finite-horizon setting from now on. 

Specifically, we base our algorithm on the  optimistic multiplicative weight updates \cite{daskalakis2018last,weilinear} and the entropy regularization technique \cite{neu2017unified} for reward functions. The algorithmic idea has been shown useful for finding $\epsilon$-approximate NE in 
two-player zero-sum MGs \cite{cen2021fast,cen2022faster}. 
{Before delving into the details of our algorithm, we introduce the notation  $\bQ_{h,i}(s)$ and $\bQ_h(s)$ as follows: 
 \begin{align*} 
     &\bQ_{ h, i}(s) := (Q_{ h, i,1}(s), \dots, Q_{h, i,i-1 }(s), \bm{0}, Q_{ h, i,i+1}(s) \dots, Q_{ h, i, n}(s)) \in  \RR^{|\cA_i| \times \sum_{i \in \cN} |\cA_i| }   
     \\     
     &\bQ_h(s) := ((\bQ_{ h,1}(s))^\intercal, (\bQ_{h,2}(s))^\intercal, \dots, (\bQ_{h,n}(s))^\intercal)^\intercal \in \RR^{\sum_{i \in \cN} |\cA_i| \times \sum_{i \in \cN} |\cA_i| }.
\end{align*}
Here, $Q_{h,i,j}$ represents an estimate of the equilibrium value function with canonical decomposition (\Cref{def:canonical}).}  Hereafter, we similarly define the notation of $\bQ_{h, i}^\pi$ and $\bQ_h^\pi$.  Our entropy-regularized OMWU algorithm contains two main steps as follows: (1) Policy update: update $\pi_{h, i}$ and $\bar{\pi}_{h, i}$ as
\begin{equation}
\begin{aligned}
  \text{Update~~~~} &\pi_{h,i}(a_i \mid s) \propto \pi_{h, i}(a_i \mid s)^{1-\eta \tau} \exp\left(\eta [ \bQ_{h, i}(s)\bar{\pi}_h (s) ]_{a_i}\right), \text{~~~~and then }
  \\
 \text{Update~~~~} &\bar{\pi}_{h, i}(a_i \mid s) \propto  \pi_{h, i}(a_i \mid s)^{1-\eta \tau} \exp\left(\eta [ \bQ_{h, i}(s)\bar{\pi}_h(s)]_{a_i}\right),
\end{aligned}
\label{eqn:omwu-updates-mainpaper}
\end{equation}
\cpdelete{(\Cref{alg:Policyopt}'s Equation \eqref{eqn::OMWUupdate1} and \eqref{eqn::OMWUupdate2})}where $\eta\geq 0$ is a step-size for the OMWU policy update and $\tau$ is the coefficient of the entropy regularization, so that $\pi_{h, i}$ and $\bar{\pi}_{h, i}$ estimate the regularized game's equilibrium policy, and (2) Value update: update each $Q_{h, i,j}$ and $V_{h, i}$ \cpdelete{with equation \eqref{eqn:Qupdates}, \eqref{eqn:Qupdates2}, and \eqref{eqn:Vupdates}}, which estimate the equilibrium value functions of the regularized game. The value update utilizes a canonical decomposition form, using value function {estimates} $V_{h, i}$ (\Cref{def:canonical}); {in particular, when $\cN_C \neq \emptyset$,  $Q_{h,i}$ and $V_{h, i}$ are {updated as follows for all $s\in\cs, a_i\in\cA_i$, and $a_j\in\cA_j$}:} 
\begin{align*}
    &Q_{h,i,j}(s, a_i, a_j) \leftarrow r_{h,i,j}(s, a_i, a_j) + \sum_{s' \in \cS} \biggl(\frac{1}{|\cE_{Q, i}|} \pmb{1}(i \in \cN_C) \FF_{h, i} (s' | s, a_i)  +  \pmb{1}(j \in \cN_C)\FF_{h, j}(s' | s,a_j)\biggr)  V_{h+1, i}(s')       
  \\
  &V_{h, i}(s) \leftarrow (1- \eta \tau)V_{h, i}(s) + \eta \tau \bigg[ \bar{\pi}_{h, i}^{\intercal}(s) \bQ_{h,i}(s) \bar{\pi}_{h}(s) +  {\tau} \cH(\bar{\pi}_{h, i}(s))  - \sum_{j \in \cE_{Q, i}}({\tau}/|\cE_{Q, i}|) \cH(\bar{\pi}_{h, j}(s))\bigg],
\end{align*}
  where 
$\eta\geq 0$ is a step-size for the OMWU policy update in step (1), $\tau$ is the coefficient of the entropy regularization, and  $\cH$ denotes the Shannon entropy function. When $\cN_C = \emptyset$, we can  similarly define updates of $Q_{h,i}$ and $V_{h,i}$.  The overall procedure is summarized in \Cref{alg:Policyopt}. 







We now state the theoretical guarantee of \Cref{alg:Policyopt} as follows. Hereafter, we will use the superscript ${(t)}$ to denote the $t$-th iteration of an iterative value within the algorithm.
\begin{restatable}{theorem}{convrate}
    \label{thm:convrate-policy-main}
    With $\eta = \frac{1}{8Hn + 1}$ and  $ \tau = \frac{\epsilon}{Hn\max_{i \in \cN} \log|\cA_i|}$, an $\epsilon$-approximate {Markov} NE of the finite-horizon MZNMG can be  attained with an iteration complexity of ${t=}\tilde{\cO}\left({H^3n}/{\epsilon}\right)$ by $\bar{\pi}{^{(t)}}$ in  \Cref{alg:Policyopt}. 
\end{restatable}

We defer a detailed proof to \Cref{appendix:OMWU}{, and provide a sketch as follows}. 
\begin{proof}[Proof Sketch of \Cref{thm:convrate-policy-main}]
{Note that for} sufficiently small $\tau>0$ {(of order $O(\epsilon)$)}, an NE of the $\tau$-regularized game  (i.e., the  quantal response equilibrium (QRE)  \cite{mckelvey1995quantal} of the original unregularized game) can approximate the NE of the original game. {Let  $(\pi_{\tau,h}^\star)_{h \in [H]}$ denote the  NE of the $\tau$-regularized MZNMG.} It thus suffices to prove that $(\pi_h^{(t)})_{t\geq 0}$ and $(\bar{\pi}_h^{(t)})_{t\geq 0}$ {in our \Cref{alg:Policyopt}} converge to $\pi_{\tau,h}^\star$ exponentially fast for every $h \in [H]$. {Define $\mathrm{KL}_s(\pi_1||\pi_2):= \mathrm{KL}(\pi_1(s) \| \pi_2(s))$.} Firstly, for the  OMWU updates \eqref{eqn:omwu-updates-mainpaper}, we can show the following
\small
\begin{align}\label{equ:proof_sketch_1}
& \mathrm{KL}_s\left(\pi_{\tau, h}^\star \| \pi_h^{(t_2)}\right)+(1-4 \eta Hn) \mathrm{KL}_s\left(\pi_h^{(t_2)} \| \bar{\pi}_{h}^{(t_2)}\right)
\\
&\leq (1-\eta \tau)^{t_2 - t_1} \left(\mathrm{KL}_s\left(\pi_{\tau, h}^\star \| \pi_h^{(t_1)}\right)  +(1 - 4\eta Hn) \mathrm{KL}_s\left(\pi_h^{(t_1)} \| \bar{\pi}_h^{(t_1)}\right)\right) + 6 \eta \sum_{l= t_1}^{t_2} (1- \eta \tau)^{t_2 - l}\sum_{i \in \cN} g\left(\bQ_{h}^{(l)}(s) - \bQ_{\tau, h}^{\pi^\star_\tau} (s), i\right)\notag
\end{align}
\normalsize
for any $0\leq t_1 < t_2$, $h \in [H]$ and $s \in \cS$ (\Cref{lem:KL-Q-relationship}), where $\bQ_{\tau, h}^{\pi_\tau^\star}$ is the $Q$-value function corresponding to the regularized NE $\pi_\tau^\star$. 
Here, $g: \RR^{\sum_{i \in \cN} |\cA_i| \times \sum_{i \in \cN} |\cA_i|}  \times \cN\to  \RR$ is  defined as 
\small
\begin{align}
    \label{equ:def_g_semi}
    g(\bQ(s),  j) = \max_{a_j \in \cA_j} \left| \left( \sum_{  k \in \cE_{Q, j} } \max_{a_k \in \cA_k} Q_{k,j}(s, a_k, a_j) \right)\right|.
\end{align}
\normalsize
{Note that $g(\cdot,\cdot)$ here can be viewed as the multi-player extension of $\norm{\cdot}_{\max}$, which was used in the proof for two-player zero-sum cases \cite{cen2022faster}. 
} 
Therefore, if we prove that $g\left(\bQ_{h}^{(t)}(s) - \bQ_{\tau, h}^{\pi^\star_\tau} (s), i\right)$ converges to 0 exponentially fast {for all $i\in\cN$}, then we can also prove by \Cref{equ:proof_sketch_1} that the KL-divergence between $\pi_{\tau, h}^\star$ and  $\pi_h^{(t)}$ converges to 0 exponentially fast. 
{To this end}, we prove another inequality 
\small
\begin{align}
    &\sum_{i \in \cN} \max_{s\in\cS} g \left(\bQ_{h-1}^{\left(t_2\right)}(s) - \bQ_{\tau, h-1}^{\pi^\star_\tau}(s), i\right) \leq 2(1-\eta \tau)^{(t_2 - t_1)}Hn^2 + 4\eta\tau \left(\sum_{t=t_1-1}^{t_2-1}(1-\eta \tau)^{t_2-1-t}\sum_{i \in \cN} \max_{s \in \cS}g\left(\bQ_{h}^{(t)}(s)- \bQ_{\tau, h}^{\pi^\star_\tau}(s), i\right)\right) \nonumber \\
    & \quad+\tau(1-\eta \tau)^{(t_2-t_1)} \max_{s \in \cS}\left(\mathrm{KL}_s\left(\pi_{\tau, h}^{\star} \| \pi_h^{\left(t_1-1\right)}\right)+(1-4 \eta Hn) \mathrm{KL}_s\left(\pi_h^{\left(t_1-1\right)} \| \bar{\pi}_h^{\left(t_1-1\right)}\right)\right)    \label{eqn:lem-boundgk}
    \end{align}
\normalsize
for any $0\leq t_1 < t_2$ and $h \in [H]$  (\Cref{lem:boundgk}). {In order to establish this inequality, we utilized a property inherent to MZNGs  (\Cref{lem:zerosum-separablesum}), for which we  refer to \Cref{rmk:technical_challenges} and \Cref{appendix:OMWU-omitted} for a more detailed explanation. Using  \Cref{eqn:lem-boundgk}, we can inductively prove that $\sum_{i \in \cN} \max_{s\in\cS} g \left(\bQ_{h-1}^{\left(t_2\right)}(s)- \bQ_{\tau, h-1}^{\pi^\star_\tau}(s), i\right)$ converges to $0$ at an exponential rate  (\Cref{thm:Qconvgnorm}), as $\mathrm{KL}_s\left(\pi_{\tau, h}^{\star},  \pi_h^{\left(t_1-1\right)}\right)$ and $\mathrm{KL}_s\left(\pi_h^{\left(t_1-1\right)} , \bar{\pi}_h^{\left(t_1-1\right)}\right)$ are bounded. Then, using \Cref{equ:proof_sketch_1} yields that $\mathrm{KL}_s\left(\pi_{\tau, h}^{\star} \| \bar{\pi}_h^{(t)}\right)$ converges to 0 at an exponential rate, and additionally we can also show that $\mathrm{KL}_s\left(\bar{\pi}_h^{(t)} \| \pi_{\tau, h}^{\star}\right)$ converges to 0 at an exponential rate (\Cref{claim:KLbound}). Lastly, we can easily show that if $\mathrm{KL}_s\left(\pi_{\tau, h}^{\star} \| \bar{\pi}_h^{(t)}\right)$ and  $\mathrm{KL}_s\left(\bar{\pi}_h^{(t)} \| \pi_{\tau, h}^{\star}\right)$ converges to 0 at an exponential rate, then the corresponding $Q$-value of $\bar{\pi}^{(t)}$ converges to the corresponding $Q$-value of $\pi_{\tau}^{\star}$ so that $\bar{\pi}^{(t)}$ converges to a Markov NE of $\tau$-regularized MZNMG (\Cref{lem::QRE-Gap2}). 
}
\end{proof}
\begin{remark}[Technical challenges]
\label{rmk:technical_challenges}
We note that some steps in the proof  follow from that for the two-player zero-sum case \cite{cen2022faster}. 
However, for the two-player zero-sum case, we have  $Q_{h, i,j}^{(l)}(s) = -Q_{h, j, i}^{(l)\intercal}(s)$ always hold for all $s \in \cS$.  {While} for  the multi-player case, $Q_{h, i,j}^{(l)}(s) \neq -Q_{h, j, i}^{(l)\intercal}(s)$ for all $s \in \cS$, and instead we have $\sum_{i \in \cN} \sum_{j \in \cE_{Q, i}} \mu_i^\intercal(s) Q_{h, i,j}^{(l)}(s) \mu_j(s) = 0$ and $\sum_{i \in \cN} \sum_{j \in \cE_{Q, i}} (\mu_i^\intercal(s) Q_{h, i,j}^{(l)}(s) \nu_j(s) + \mu_j^\intercal(s) Q_{h, i,j}^{(l) \intercal}(s) \nu_i(s)) = 0$ for arbitrary policies $\mu$ and $\nu$ (\Cref{lem:zerosum-separablesum}, \cite{leonardos2021exploration,ao2022asynchronous}). We have to properly exploit this property.
For example, \Cref{lem:boundgk}, {which bounds  the difference between the $Q$-value estimates and {the equilibrium $Q$-value of the  regularized game,}} cannot hold if we do not have {a} summation over $i$. To be specific, we can write $ \sum_{i \in \cE_{Q, j} } \langle  \bar{\pi}_{h,j}^{(l)}(s) - \pi_{h,j}^{(l)}(s), - Q_{h,j, i}^{(l-1)}(s)\bar{\pi}_{h, i}^{(l-1)}(s)  \rangle$ (\circled{1}) as a summation  of KL divergence. However, if we analyze it without summing over $i$, we need to analyze $\sum_{j \in \cE_{Q, i}} \langle\bar{\pi}_{h,j}^{(l)}(s)-{\pi}_{h,j}^{(l)}(s), Q_{h, i,j}^{(l-1) \intercal}(s) \bar{\pi}_{h,i}^{(l-1)}(s)\rangle$ (\circled{2}). If there are only two players, these two formulas would be identical  since there is only one element for the summation, and  we can also directly use $Q_{h,i,j}^{(l-1)\intercal}(s) = -Q_{h, j, i}^{(l-1)}(s)$ (\circled{3}) as \cite{cen2022faster} did. However, without \circled{3}, {\circled{2} is not identical to \circled{1}. After summing over $i$ of \circled{2}, and changing the order of summation, we still cannot easily bound the summation of \circled{2} over players} since it has {a}  $Q^\intercal$ term,  which inspires us to make a  new use of \Cref{lem:zerosum-separablesum} {to  calculate the  summation regarding $Q^\intercal$}. 
Moreover, {to facilitate our analysis,} we defined a new measure 
$g(\cdot, \cdot)$ (c.f. \Cref{equ:def_g_semi}) {that might  be of independent interest},  which allows us to analyze the sum of $Q$ values, while \cite{cen2022faster} used norm as $\norm{\cdot}_{\max}$, which,  in multi-player cases, may not be controlled properly. 
\end{remark}


  



==> main7-QRE.tex <==
\chapter{Smooth Q-learning and Uniqueness of Quantal Response Equilibrium}
\label{sec:smoothq}

Smooth Q-learning \cite{tuyls2003selection, sato2003coupled} is a well-known variant of Q-learning \cite{watkins1992q}. This variant incorporates softmax exploration into its framework, which can be defined mathematically as follows: for each agent $i$
\begin{equation}
\begin{aligned}
    &q_i^{(k+1)}(s, a_i) = q_i^{(k)}(s, a_i) + \alpha_i\left(Q_{i}^{\pi^{(k)}}(s, a_i, \pi_{-i}^{(k)}) - q_i^{(k)}(s, a_i)\right)
    \\
    & \pi_i^{(k+1)}(a_i \mid s) = \frac{\exp\left(q_i^{(k+1)}(s, a_i)/\tau_i\right)}{\sum_{a_i' \in \cA_i}\exp\left(q_i^{(k+1)}(s, a_i')/\tau_i\right)} 
\end{aligned}
\tag{Q-learning discrete version}  \label{eqn:q-learning-discrete}
\end{equation}
for all $s \in \cS, a_i \in \cA_i$
where  $q_i^{(k)} \in \RR^{|\cS| \times |\cA_i|}, \pi_i^{(k)} \in \RR^{|\cS| \times |\cA_i|}$, $k \geq 0$ denotes timesteps, $\alpha_i$ is the learning rate of agent $i$, and $\tau_i>0$ is a temperature parameter, which represents the degree of the bounded rationality of the agent $i$. Here, $\pi_{-i}^{(k)}(\ba_{-i} \mid s):= \prod_{j \neq i} \pi_j^{(k)} (a_j \mid s)$, $\PP(s'\mid s, a_i, \pi_{-i}^{(k)}):= \sum_{\ba_{-i} \in \cA_{-i}} \PP(s'\mid s, a_i, \ba_{-i})\pi_{-i}^{(k)}( \ba_{-i} \mid s)$, and  $Q_i^{\pi^{(k)}}(s, a_i, \pi_{-i}^{(k)}) := \sum_{\ba_{-i} \in \cA_{-i}} \pi_{-i}^{(k)} (\ba_{-i}\mid  s) Q_i^{\pi^{(k)}} (s, \ba) = r(s, a_i,\pi_{-i}^{(k)}) + \gamma \PP(s'\mid s, a_i, \pi_{-i}^{(k)}) V_i^{\pi^{(k)}}(s')$. 
Now, we will analyze the continuous version of the (\ref{eqn:q-learning-discrete}) as follows: 
\begin{equation}
\begin{aligned}
    &\dot{q_i}(s, a_i) =  \alpha_i\left(Q_{i}^{\pi}(s, a_i, \pi_{-i}) - q_i(s, a_i)\right)
    \\
    & \pi_i(a_i \mid s) = \frac{\exp\left(q_i(s, a_i)/\tau_i\right)}{\sum_{a_i' \in \cA_i}\exp\left(q_i(s, a_i')/\tau_i\right)} 
\end{aligned}
\tag{Q-learning continuous version}  \label{eqn:q-learning-continuous}
\end{equation}
\begin{equation}
\begin{aligned}
    &\dot{q_i}(s, a_i) =  \alpha_i\left(Q_{{\color{blue}\tau}, i}^{\pi}(s, a_i, \pi_{-i}) - q_i(s, a_i)\right)
    \\
    & \pi_i(a_i \mid s) = \frac{\exp\left(q_i(s, a_i)/\tau_i\right)}{\sum_{a_i' \in \cA_i}\exp\left(q_i(s, a_i')/\tau_i\right)} 
\end{aligned}
\tag{$Q_\tau$-learning continuous version}  \label{eqn:q-learning-continuous}
\end{equation}


for all $s \in \cS, a_i \in \cA_i$.
\begin{proposition}
Assume that players follow the dynamics of (\ref{eqn:q-learning-continuous}). Then, the evolution of $\pi_i$ can be represented as 
\begin{equation}
\begin{aligned}
    \dot{\pi}_i(a_i \mid s) = \frac{\alpha_i}{\tau_i}{\pi}_i(a_i \mid s) \Bigg(Q_i^\pi(s, a_i, \pi_{-i})& - \sum_{a_i' \in \cA_i} \pi_i(a_i' \mid s) Q_i^\pi(s, a_i', \pi_{-i})
    \\
    &- \tau_i \Bigl(\ln \pi_i(a_i \mid s) - \sum_{a_i' \in \cA_i} \pi(a_i' \mid s) \ln \pi_i(a_i' \mid s) \Bigr)\Biggr)
\end{aligned} \label{eqn:pi-evolution}    
\end{equation}
for all $i \in \cN, s \in \cS, a_i \in \cA_i$. 

\end{proposition}
\begin{proof}
    The proof is similar to \cite{leonardos2021exploration}, and also a similar calculation can be found in \cite{galla2013complex, sato2005stability, kianercy2012dynamics, tuyls2003selection, sato2003coupled}. The time derivative of $\pi_i(a_i \mid s)$ is 
    \begin{align*}
        &\dot{\pi}_i(a_i \mid s) = \frac{\exp\left(q_i(s, a_i)/\tau_i\right)}{\tau_i \sum_{a_i' \in \cA_i}\exp\left(q_i(s, a_i')/\tau_i\right)} \left(\dot{q}_i(s, a_i) - \frac{\sum_{a_i' \in \cA_i} \dot{q}_i(s, a_i') \exp({q}_i(s, a_i')/\tau_i)}{\sum_{a_i' \in \cA_i} \exp({q}_i(s, a_i')/\tau_i)}\right)
        \\
        &= \frac{1}{\tau_i} {\pi}_i(a_i \mid s)\left(\dot{q}_i(s, a_i) - \sum_{a_i' \in \cA_i} \pi_i(a_i' \mid s) \dot{q}_i(s, a_i')\right)
        \\
        &\underset{(i)}{=} \frac{\alpha_i}{\tau_i} {\pi}_i(a_i \mid s)\left(Q_i^\pi(s, a_i, \pi_{-i}) -{q}_i(s, a_i) - \sum_{a_i' \in \cA_i} \pi_i(a_i' \mid s) ( Q_i^\pi(s, a_i', \pi_{-i}) - {q}_i(s, a_i'))\right)
        \\
        &\underset{(ii)}{=} \frac{\alpha_i}{\tau_i}{\pi}_i(a_i \mid s) \Bigg(Q_i^\pi(s, a_i, \pi_{-i}) - \sum_{a_i' \in \cA_i} \pi_i(a_i' \mid s) Q_i^\pi(s, a_i', \pi_{-i}) 
        \\
        &\qquad \qquad \qquad \qquad - \tau_i \Bigl(\ln \pi_i(a_i \mid s) - \sum_{a_i' \in \cS} \pi_i(a_i' \mid s) \ln \pi_i(a_i' \mid s) \Bigr)\Biggr)
    \end{align*}
    where $(i)$ comes from $\dot{q_i}(s, a_i) =  \alpha_i\left(Q_{i}^{\pi}(s, a_i, \pi_{-i}) - q_i(s, a_i)\right)$ and $(ii)$ comes from $\pi_i(a_i \mid s) = \frac{\exp\left(q_i(s, a_i)/\tau_i\right)}{\sum_{a_i' \in \cA_i}\exp\left(q_i(s, a_i')/\tau_i\right)}$. 
\end{proof}

\begin{definition}[(Stationary) Quantal Response Equilibrium]
    A (stationary) Quantal Response Equilibrium (QRE) $\pi^\star \in \left(\prod_{i \in \cN} \Delta(\cA_i)\right)^{|\cS|}$ is defined as follows:
    \begin{align}
        \pi_i^\star(a_i \mid s) = \frac{\exp\left(Q_i^{\pi^\star}(s, a_i, \pi^\star_{-i}) / \tau_i \right)}{\sum_{a_i' \in \cA_i} \exp\left(Q_i^{\pi^\star}(s, a_i', \pi^\star_{-i}) / \tau_i \right)}. \label{eqn:qre2}
    \end{align}
    for all $ i \in \cN, s \in \cS, a_i \in \cA_i$. 
    \cp{check slack for the issue}
\end{definition}
We will omit ``stationary'' in this section if the meaning is clear.
\begin{proposition}
\label{prop:fixed-point-equation}
    The set of interior fixed points of \Cref{eqn:pi-evolution} is the same as the set of QRE. In other words, \Cref{eqn:qre2} is equivalent to 
        \begin{align}
        Q_i^{\pi^\star}(s, a_i, \pi^\star_{-i}) &- \sum_{a_i' \in \cA_i} \pi^\star_i(a_i' \mid s) Q_i^{\pi^\star}(s, a_i', \pi^\star_{-i}) \nonumber
        \\
        &- \tau_i \Bigl(\ln \pi^\star_i(a_i \mid s) - \sum_{a_i' \in \cS} \pi^\star_i(a_i' \mid s) \ln \pi^\star_i(a_i' \mid s) \Bigr) = 0,  \label{eqn:QRE}
    \end{align}
    for all $i \in \cN$, $s \in \cS$, and $a_i \in \cA_i$. Plus, QRE always exists for any MG. Lastly, for arbitrary $\pi \in \left(\prod_{i \in \cN} \Delta(\cA_i)\right)^{|\cS|}$, \begin{align*}
        (\pi_i(s) - \pi_i^\star(s))^\intercal (Q_i^{\pi^\star}(s, \pi_{-i}^\star) - \tau_i \ln (\pi_i^\star(s))) = 0.
    \end{align*}
\end{proposition}
\begin{proof}
    Applying $\ln$ function to the both side of \Cref{eqn:qre2}, we have 
    \begin{align*}
        \ln \pi_i^\star(a_i \mid s) = Q_i^{\pi^\star}(s, a_i, \pi^\star_{-i}) / \tau_i - \ln \sum_{a_i' \in \cA_i} \exp\left(Q_i^{\pi^\star}(s, a_i', \pi^\star_{-i}) / \tau_i \right)
    \end{align*}    
    for all $i \in \cN$, $a_i \in \cA_i$ and $s \in \cS$. Therefore, we have 
    \begin{align*}
        \sum_{a_i \in \cA_i} \pi^\star_i(a_i \mid s) \ln \pi_i^\star(a_i \mid s) &= \sum_{a_i \in \cA_i} \pi^\star_i(a_i \mid s) Q_i^{\pi^\star}(s, a_i, \pi^\star_{-i}) / \tau_i 
        \\
        &\qquad -  \ln \sum_{a_i' \in \cA_i} \exp\left(Q_i^{\pi^\star}(s, a_i', \pi^\star_{-i}) / \tau_i \right)
\end{align*}
which proves that QREs are the fixed point of \Cref{eqn:pi-evolution}. The opposite direction can be proved similar with \cite[Theorem 3.2]{leonardos2021exploration}.  Plus, since $Q^\pi_i$ is a continuous function \cite{agarwal2019reinforcement}, by the Brouwer fixed point theorem\kz{ref}, there exists a $\pi^\star$ that satisfies \Cref{eqn:QRE}.  Plus, for arbitrary $\pi \in \left(\prod_{i \in \cN} \Delta(\cA_i)\right)^{|\cS|}$, summing \Cref{eqn:QRE} with multiplying $\pi_i(a_i \mid s)$ for all $a_i \in \cA_i$ provides \cp{check here please}
    \begin{align*}
        (\pi_i(s) - \pi_i^\star(s))^\intercal (Q_i^{\pi^\star}(s, \pi_{-i}^\star) - \tau_i \ln (\pi_i^\star(s))) = 0.
    \end{align*}
\end{proof}
In sum, QREs are the interior fixed points of (\ref{eqn:q-learning-continuous}). 





\begin{fact}
\label{fact:KL-sum}
    For any $\mu, \nu \in \Delta(\cA_i)$, \begin{align*}
        \KL(\mu \| \nu) + \KL(\nu \| \mu) = (\mu - \nu)^\intercal(\ln(\mu) - \ln(\nu)). 
    \end{align*} 
\end{fact}

\begin{lemma}
 For \textbf{any} QRE $\pi^\star$, we have 
 \begin{equation}
\begin{aligned}
\frac{d}{d t} \KL\left(\pi^\star_i(s) \| \pi_i (s) \right)&=\frac{\alpha_i}{\tau_i}\left(\pi_i(s)-\pi^\star_i(s) \right)^{\top}\left(Q_i^{\pi}\left(s, \pi_{-i}\right)-Q_i^{\pi^\star}\left(s, \pi^\star_{-i}\right)\right)
\\
&\qquad \qquad -\alpha_i\left(\KL\left(\pi^\star_i(s) \| \pi_i (s)\right)+\KL\left(\pi_i(s) \| \pi^\star_i(s)\right)\right)    
\end{aligned}
\label{eqn:KL-derivative}     
 \end{equation}
 for any $i \in \cN$ and $s \in \cS$.
\end{lemma}
\begin{proof}
The time derivative of the term $\KL\left(\pi^\star_i \| \pi_i\right)$ for $k \in \cN$ can be calculated as follows (note that after the first line, we omit the dependence of $\pi$ on $t$ to simplify notation)
$$
\begin{aligned}
\frac{d}{d t}& \KL\left(\pi^\star_i (s) \| \pi_i(s)\right)  =-\sum_{a_i \in \cA_i} \pi^\star_i(a_i \mid s) \frac{d}{d t}\left(\ln \left(\pi_i(a_i \mid s)\right)\right)=-\sum_{a_i \in \cA_i} \pi^\star_i(a_i \mid s) \frac{\dot{\pi}_i(a_i \mid s)}{\pi_i(a_i \mid s)} \\
& =-\sum_{a_i \in \cA_i} \pi^\star_i(a_i \mid s)\Biggl(\frac{\alpha_i}{\tau_i}\Bigg(Q_i^\pi(s, a_i, \pi_{-i}) - \sum_{a_i' \in \cA_i} \pi_i(a_i' \mid s) Q_i^\pi(s, a_i', \pi_{-i}) 
\\
&\qquad \qquad \qquad \qquad \qquad \qquad - \tau_i \Bigl(\ln \pi_i(a_i \mid s) - \sum_{a_i' \in \cA_i} \pi(a_i' \mid s) \ln \pi_i(a_i' \mid s) \Bigr)\Biggr) \Biggr)  \\
& =-\frac{\alpha_i}{\tau_i} \left(\pi^{\star\top}_i(s) Q_i^\pi \left(s, \pi_{-i}\right)-\pi_i^{\top}(s) Q_i^\pi\left(s, \pi_{-i}\right)+\tau_i\left(-\pi^{\star\top}_i(s) \ln \left(\pi_i(s)\right)+\pi_i^{\top}(s) \ln \left(\pi_i(s)\right)\right)\right) \\
& =\frac{\alpha_i}{\tau_i}\left(\pi_i(s)-\pi^\star_i(s)\right)^{\top}\left(Q_i^\pi\left(s, \pi_{-i}\right)-\tau_i \ln \left(\pi_i(s)\right)\right) 
\\
& \underset{(i)}{=}\frac{\alpha_i}{\tau_i}\left(\pi_i(s)-\pi^\star_i(s)\right)^{\top}\left(Q_i^\pi\left(s, \pi_{-i}\right)-Q_i^{\pi^\star}(s, \pi_{-i}^\star) - \tau_i (\ln \left(\pi_i(s)\right) - \ln (\pi_i^\star(s))) \right) 
\\
&\underset{(ii)}{=} \frac{\alpha_i}{\tau_i}\left(\pi_i(s)-\pi^\star_i(s)\right)^{\top}\left(Q_i^\pi\left(s, \pi_{-i}\right)-Q_i^{\pi^\star}(s, \pi_{-i}^\star)\right) - \alpha_i \left( \KL\left(\pi^\star_i \| \pi_i\right)+\KL\left(\pi_i \| \pi^\star_i\right) \right) 
\end{aligned}
$$
where $(i)$ holds due to \Cref{prop:fixed-point-equation} and $(ii)$ holds due to \Cref{fact:KL-sum}.
\end{proof}

\begin{claim}
    For zero-sum NMG $(\cG = (\cN, \cE_Q), \cS, \cA, \PP, (r_{i})_{i \in \cN}, \gamma)$,
    \begin{align*}
        \sum_{i \in \cN}\left(\pi_i(s)-\pi^\star_i(s)\right)^{\top}\left(Q_i^\pi\left(s, \pi_{-i}\right)-Q_i^{\pi^\star}(s, \pi_{-i}^\star)\right) = 0
    \end{align*}
    holds for any $s \in \cS$.
\end{claim}

\begin{proof}
    \begin{align*}
        &\sum_{i \in \cN}  \left(\pi_i(s)-\pi^\star_i(s)\right)^{\top}\left(Q_i^\pi\left(s, \pi_{-i}\right)-Q_i^{\pi^\star}(s, \pi_{-i}^\star)\right)
        \\
        &=\sum_{i \in \cN}  \left(\pi_i(s)-\pi^\star_i(s)\right)^{\top}\left(Q_i^\pi\left(s, \pi_{-i}\right)- Q_i^\pi(s, \pi_{-i}^\star) +Q_i^\pi(s, \pi_{-i}^\star) -  Q_i^{\pi^\star}(s, \pi_{-i}^\star)\right)
        \\
        &\underset{(i)}{=}\sum_{i \in \cN}  \left(\pi_i(s)-\pi^\star_i(s)\right)^{\top}\left(Q_i^\pi(s, \pi_{-i}^\star) -  Q_i^{\pi^\star}(s, \pi_{-i}^\star)\right)
        \\
        &=\sum_{i \in \cN} \sum_{a_i \in \cA_i}  \left(\pi_i(a_i \mid s)-\pi^\star_i(a_i \mid s)\right)\Biggl( \gamma\sum_{s' \in \cS} \PP(s'\mid s, a_i, \pi_{-i}^\star) V_i^{\pi}(s') - \gamma\sum_{s' \in \cS} \PP(s'\mid s, a_i, \pi^\star_{-i}) V_i^{\pi^\star}(s')  \Biggr) 
        \\
        &= \sum_{i \in \cN} \sum_{a_i \in \cA_i} \sum_{s' \in \cS} \gamma \left(\pi_i(a_i \mid s)-\pi^\star_i(a_i \mid s)\right) \left(\PP(s'\mid s, a_i, \pi_{-i}^\star) V_i^{\pi}(s') -  \PP(s'\mid s, a_i, \pi^\star_{-i}) V_i^{\pi^\star}(s') \right)
        \\
        &\underset{(ii)}{=} \sum_{i \in \cN} \sum_{a_i \in \cA_i} \sum_{s' \in \cS} \gamma \left(\pi_i(a_i \mid s)-\pi^\star_i(a_i \mid s)\right) \left(\sum_{j \neq i} \left(\FF_j(s'\mid s, \pi_j^\star) V_i^{\pi}(s') -  \FF_j(s'\mid s, \pi_j^\star) V_i^{\pi^\star}(s')\right) \right)
        \\
        &= 0.
    \end{align*}
    \cp{check here please, I changed accordingly.}

    Here, $(i)$ came from the fact that $Q_i^\pi(s)$ form a zero-sum NG $(\cG = (\cN, \cE_Q), \cA, (Q_{i}^\pi)_{i \in \cN})$ and $(ii)$ came from the fact that $\PP(s'\mid s, \ba) = \sum_{i \in \cN} \FF_i(s'\mid s, a_i)$.
\end{proof}
Therefore, if we sum \Cref{eqn:KL-derivative} with multiplying $\frac{ \tau_i}{\alpha_i}$, we have 
\begin{align*}
    \frac{d}{dt}\sum_{i \in \cN} \frac{\tau_i}{\alpha_i}\KL\left(\pi^\star_i(s) \| \pi_i (s) \right)&= - \sum_{i \in \cN} { \tau_i}\left(\KL\left(\pi^\star_i(s) \| \pi_i (s)\right)+\KL\left(\pi_i(s) \| \pi^\star_i(s)\right)\right) 
    \\
    &\leq - \sum_{i \in \cN} { \tau_i}\KL\left(\pi^\star_i(s) \| \pi_i (s)\right) \leq -\min_{k \in \cN}\alpha_i\sum_{i \in \cN} \frac{ \tau_i}{\alpha_i}\KL\left(\pi^\star_i(s) \| \pi_i (s)\right), 
\end{align*}
which proves that $\sum_{i \in \cN} \frac{\tau_i}{\alpha_i}\KL\left(\pi^\star_i(s) \| \pi_i (s) \right)$ decreases exponentially to 0. As a byproduct, every $\pi_i(s)$ converge to any $\pi_i^\star$\kz{why this sentence gives uniqueness? why cannot it be a path-dependent/initialization-dependent convergent point? or, if we start from some $\pi^*$, it would just stay there?}\cp{because it converges to ``any'' QRE, which means that QRE should be unique}, which indicates $\pi_i^\star$ is unique.  































